Canonical Decompositions of 3-Connected Graphs

We offer a new structural basis for the theory of 3-connected graphs, providing a unique decomposition of every such graph into parts that are either quasi 4-connected, wheels, or thickened $K_{3,m}$'s. Our construction is explicit, canonical, and has the following applications: we obtain a new theorem characterising all finite Cayley graphs as either essentially 4-connected, cycles, or complete graphs on at most four vertices, and we provide an automatic proof of Tutte's wheel theorem.

==> 1Preamble.tex <==
\newcommand{\jaf}[3]{#2} % 1: Math-Journal; 2: arXiv; 3: FOCS

\input{minimalJ}

\usepackage{etoolbox} % for '\patchcmd' macro

% Leader dots in toc
\makeatletter
%\renewcommand\@pnumwidth{1em} % <-- depending on the total number of pages
\patchcmd{\@tocline}
  {\hfil}
  {\leaders\hbox{\,.\,}\hfil}
  {}{}
\makeatother

%\DeclareRobustCommand{\SkipTocEntry}[5]{} 

\usepackage{tocloft}% to configure the ToC <<<<<
\setlength{\cftsecnumwidth}{5ex}
\setlength{\cftsubsecnumwidth}{7ex}
\setcounter{tocdepth}{1}

%\documentclass[11pt]{article}


\usepackage{verbatim}
\usepackage{enumitem}
\usepackage[all]{xy}
\usepackage{subfig}
\usepackage{footnote}
\makesavenoteenv{tabular}



\newcommand{\eps}{\varepsilon}
\newcommand{\plus}{${}^+$}

\setenumerate{label={\textnormal{(\arabic*)}}}

\makeatletter
\newcommand{\dotminus}{\mathbin{\text{\@dotminus}}}

\newcommand{\@dotminus}{%
  \ooalign{\hidewidth\raise1.2ex\hbox{.}\hidewidth\cr$\m@th-$\cr}%
}
\makeatother

% new \oset macro:
\makeatletter
\newcommand{\oset}[3][0ex]{%
  \mathrel{\mathop{#3}\limits^{
    \vbox to#1{\kern-0.1\ex@
    \hbox{$\scriptstyle#2$}\vss}}}}
\makeatother

\theoremstyle{plain}
\newtheorem{main}{Theorem}
\def\mainautorefname{Theorem}
\newcommand{\mainmize}[2]{\newaliascnt{#1}{main} \newtheorem{#1}[#1]{#2} \aliascntresetthe{#1}}
\mainmize{mcor}{Corollary}
\def\mcorautorefname{Corollary}

\newtheorem{innercustomthm}{}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
  
\newtheorem{innercustomcor}{}
\newenvironment{customcor}[1]
  {\renewcommand\theinnercustomcor{#1}\innercustomcor}
  {\endinnercustomcor}
\def\customcorautorefname{Corollary}

\usepackage{xcolor}
\colorlet{darkishRed}{red!80!black}
\colorlet{darkishBlue}{blue!60!black}
\colorlet{darkishGreen}{green!60!black}
%\hypersetup{
%    draft = false,
%    bookmarksopen=true,
%    colorlinks,
%    linkcolor={red!60!black},
%    citecolor={green!60!black},
%    urlcolor={blue!60!black}
%}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\green}[1]{{\color{darkishGreen}{#1}}}
\newcommand{\todo}[1]{{\color{darkishGreen}{#1}}}

\newcommand{\sm}{\setminus}

\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\ge}{\geqslant}
\newcommand{\ty}[1]{{\tt#1}}
\DeclareMathOperator{\expl}{Ex_r}
\DeclareMathOperator{\degree}{deg}
\DeclareMathOperator{\cons}{cons}
\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\Br}{Br}
\DeclareMathOperator{\Sbb}{\mathbb{S}}

%\usepackage[notref,notcite]{showkeys}
\newcommand{\ct}{^\complement}

\newcommand{\Sthree}{$\Sbb^3$}

\mcm{\Fbb}{0}{\mathbb{F}}

\def\lowfwd #1#2#3{{\mathop{\kern0pt #1}\limits^{\kern#2pt\raise.#3ex
\vbox to 0pt{\hbox{$\scriptscriptstyle\rightarrow$}\vss}}}}
\def\lowbkwd #1#2#3{{\mathop{\kern0pt #1}\limits^{\kern#2pt\raise.#3ex
\vbox to 0pt{\hbox{$\scriptscriptstyle\leftarrow$}\vss}}}}
\def\fwd #1#2{{\lowfwd{#1}{#2}{15}}}
\def\Sinf{S_{\aleph_0}}
\def\SinfT{\Sinf^{\,\normalfont\text{t}}}
\def\vS{{\hskip-1pt{\fwd S3}\hskip-1pt}}
\def\vSinf{\vS_{\mkern-.85\thinmuskip\aleph_0}}
\def\vSinfT{\vS{}{}_{\aleph_0}^{\,\normalfont\text{t}}}
\def\vE{{\hskip-1pt{\fwd{E}{3.5}}\hskip-1pt}}
\def\vF{{\hskip-1pt{\fwd{F}{3.5}}\hskip-1pt}}
\def\ve{\kern-1.5pt\lowfwd e{1.5}2\kern-1pt}
\def\ev{\kern-1pt\lowbkwd e{0.5}2\kern-1pt}
\def\vf{\kern-2pt\lowfwd f{2.5}2\kern-1pt}
\def\fv{\lowbkwd f01}
\def\vT{\lowfwd T{0.3}1}
\def\vs{\lowfwd s{1.5}1}%1.5
\def\sv{\lowbkwd s{0}1}


==> minimalJ.tex <==
% This is my basic toolkit; things I will always want.

% First, some packages:
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsbsy}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{textcomp}
\usepackage{hyperref}
\usepackage{aliascnt}
\usepackage{mathrsfs}

% Then, some commands I'll need:
% Nicked  from Leinster:
\newcommand{\mcm}[3]{\newcommand{#1}[#2]{{\ensuremath{#3}}}} 
\newcommand{\cay}{\textnormal{Cay}}
\mcm{\tuple}{1}{\langle #1 \rangle}
\mcm{\name}{1}{\ulcorner #1 \urcorner}
\mcm{\Nbb}{0}{\mathbb{N}}
\mcm{\Zbb}{0}{\mathbb{Z}}
\mcm{\Rbb}{0}{\mathbb{R}}
\mcm{\Cbb}{0}{\mathbb{C}}
\mcm{\Qbb}{0}{\mathbb{Q}}
\mcm{\Acal}{0}{\mathcal A}
\mcm{\Bcal}{0}{\mathcal B}
\mcm{\Ccal}{0}{\mathcal C}
\mcm{\Dcal}{0}{\mathcal D}
\mcm{\Ecal}{0}{\mathcal E}
\mcm{\Fcal}{0}{\mathcal F}
\mcm{\Gcal}{0}{\mathcal G}
\mcm{\Hcal}{0}{\mathcal H}
\mcm{\Ical}{0}{\mathcal I}
\mcm{\Jcal}{0}{\mathcal J}
\mcm{\Kcal}{0}{\mathcal K}
\mcm{\Lcal}{0}{\mathcal L}
\mcm{\Mcal}{0}{\mathcal M}
\mcm{\Ncal}{0}{\mathcal N}
\mcm{\Ocal}{0}{{\mathcal O}}
\mcm{\Pcal}{0}{{\mathcal P}}
\mcm{\Qcal}{0}{{\mathcal Q}}
\mcm{\Rcal}{0}{{\mathcal R}}
\mcm{\Scal}{0}{{\mathcal S}}
\mcm{\Tcal}{0}{{\mathcal T}}
\mcm{\Ucal}{0}{{\mathcal U}}
\mcm{\Vcal}{0}{{\mathcal V}}
\mcm{\Wcal}{0}{{\mathcal W}}
\mcm{\Xcal}{0}{{\mathcal X}}
\mcm{\Ycal}{0}{{\mathcal Y}}
\mcm{\Zcal}{0}{{\mathcal Z}}
\mcm{\Mfrak}{0}{\mathfrak M}
\newcommand{\easy}{\nobreak\hfill$\square$\medskip}
\newcommand{\contradiction}{\nobreak\hfill\textreferencemark\medskip}
\DeclareMathOperator{\Cl}{Cl}
\mcm{\restric}{0}{\upharpoonright}
\mcm{\upset}{0}{\uparrow}
\mcm{\onto}{0}{\twoheadrightarrow}
\mcm{\smallNbb}{0}{{\small \mathbb{N}}}
\DeclareMathOperator{\preop}{op}
\mcm{\op}{0}{^{\preop}}
\newcommand{\supth}{\textsuperscript{th}}
\newcommand{\supst}{\textsuperscript{st}}
\newcommand{\supnd}{\textsuperscript{nd}}
\newcommand{\itum}{\item[$\bullet$]}
\newcommand{\se}{\subseteq}
%I like this environment, which is one of Leinster's:
\newenvironment{centredpic}%
{\begin{array}{c}
\setlength{\unitlength}{1em}}%
{\end{array}}

%Finally, I'll want the following theorem structure:
\usepackage{amsthm}
\renewcommand{\thesection}{\thechapter.\arabic{section}}
\newcommand{\tn}{externally 2-connected}
\newcommand{\N}{\mathbb{N}}
\newcommand{\vS}{\vec{S}}
\newcommand{\vN}{\vec{N}}
\newcommand{\cC}{\mathscr{C}}
\newcommand{\cD}{\mathscr{D}}
\newenvironment{cproof}{\noindent\textit{Proof of Claim.}}{\phantom{!}\!\hfill$\diamondsuit$}


\newcommand{\theoremize}[2]{\newaliascnt{#1}{thm} \newtheorem{#1}[#1]{#2} \aliascntresetthe{#1}}

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\theoremize{lem}{Lemma}
\theoremize{skolem}{Skolem}
\theoremize{fact}{Fact}
\newtheorem{sublem}{Claim}[thm]
\theoremize{obs}{Observation}
\theoremize{prop}{Proposition}
\theoremize{cor}{Corollary}
\theoremize{que}{Question}
\theoremize{oque}{Open Question}
\theoremize{oprob}{Open Problem}
\theoremize{con}{Conjecture}
\theoremize{setting}{Setting}

\theoremstyle{definition}
\theoremize{dfn}{Definition}
\newtheorem*{tridfn}{Definition}
\theoremize{rem}{Remark}
\theoremize{eg}{Example}
\theoremize{exercise}{Exercise}
\theoremstyle{plain}

\def\subsubsectionautorefname{Subsubsection}
\def\subsectionautorefname{Section}
\def\thmautorefname{Theorem}
\def\lemautorefname{Lemma}
\def\settingautorefname{Setting}
\def\skolemautorefname{Skolem}
\def\factautorefname{Fact}
\def\sublemautorefname{Claim}
\def\remautorefname{Remark}
\def\obsautorefname{Observation}
\def\propautorefname{Proposition}
\def\corautorefname{Corollary}
\def\queautorefname{Question}
\def\oqueautorefname{Open Question}
\def\oprobautorefname{Open Problem}
\def\conautorefname{Conjecture}
\def\dfnautorefname{Definition}
\def\egautorefname{Example}
\def\exerciseautorefname{Exercise}
\def\sectionautorefname{Section}
\def\figureautorefname{Figure}
\def\tableautorefname{Table}
\def\chapterautorefname{Chapter}


\newcommand{\myref}[1]{\autoref{#1}~(\nameref{#1})}
